A Notion of Individual Fairness for Clustering

A common distinction in fair machine learning, in particular in fair classification, is between group fairness and individual fairness. In the context of clustering, group fairness has been studied extensively in recent years; however, individual fairness for clustering has hardly been explored. In this paper, we propose a natural notion of individual fairness for clustering. Our notion asks that every data point, on average, is closer to the points in its own cluster than to the points in any other cluster. We study several questions related to our proposed notion of individual fairness. On the negative side, we show that deciding whether a given data set allows for such an individually fair clustering in general is NP-hard. On the positive side, for the special case of a data set lying on the real line, we propose an efficient dynamic programming approach to find an individually fair clustering. For general data sets, we investigate heuristics aimed at minimizing the number of individual fairness violations and compare them to standard clustering approaches on real data sets.

==> Indi Fairness - Arxiv/discussion.tex <==
In this work we 
%initiated 
contributed to 
the study of individual fairness in the context of clustering, which is only in its infancy. 
We proposed a notion of individual fairness that aims at data points being well represented by their clusters. 
Formally, it asks that every data
point, on average, is closer to the points in its own
cluster than to the points in any other cluster. 
This notion raises numerous questions, some of which we addressed: we showed that for general data sets, it is NP-hard to decide whether an individually fair $k$-clustering exists. 
In contrast, for one-dimensional Euclidean data sets we can compute a fair clustering by means of an efficient dynamic programming approach.
We examined standard clustering algorithms 
and saw that 
$k$-means++ 
often produces clusterings that are only slightly unfair. We also studied a simple heuristic to make linkage clustering more fair. 


Still, many questions remain open, and we hope to inspire follow-up work to address some of these: using our measures $\Nrunf$ or $\Maxviol$ 
(cf. Section~\ref{section_experiments}), or some other measure, to define a notion of ``approximate individual fairness'', can we design 
%approximation 
algorithms with provable guarantees for finding such an approximately fair clustering? 
Can we do so for general data sets, or which assumptions about the data set do we need to make? 
Are there classes of data sets other than 1-dimensional Euclidean 
ones 
that 
allow for a (strictly) individually fair clustering? 
Finally, can we provide guarantees for Euclidean data sets and $k$-means++ clustering, which performed surprisingly well in our experiments? 


==> Indi Fairness - Arxiv/experiments.tex <==
%In this section we present a number of experiments. 
We first study the case of 
%a
1-dim Euclidean data, 
%set, 
%in which case 
where 
we can 
% compute 
% %individually 
% fair 
% clusterings with 
% %the 
apply 
our 
%dynamic programming 
DP 
approach 
%proposed in 
of
%that we proposed in 
Section~\ref{section_1dim}.  
%
We then deal with general data sets. 
In this case, 
individually 
fair clusterings in the strict sense of Definition~\ref{def_indi_fairness}, 
which are required to treat every data point fair, may not  
exist, and 
even 
if they 
%exist,
do, 
%according to our results of Section~\ref{section_np_hardness}, 
there is no efficient way to compute them (cf. Section~\ref{section_np_hardness}).    
Hence, we have to settle for approximate versions of Definition~\ref{def_indi_fairness} and fall back on approximation algorithms 
%and 
or 
heuristics.
%
As a starting~point~for~a~study of ``approximate individual fairness'' and a thorough search for 
approximation 
algorithms~with~guarantees 
(cf. Section~\ref{section_discussion}),~we~investigate the extent to which standard clustering algorithms 
violate 
individual fairness
and 
consider 
a heuristic approach 
for finding approximately fair~clusterings. 
%
Our experiments are intended to  serve as a proof of concept.
%and to examine our proposed notion of individual fairness. 
They do not focus on the running times of the 
%various 
algorithms or their applicability to \emph{large} data sets. Hence,  
%in our experiments 
we 
only 
use rather small data sets of sizes 500~to~1885. 


Let us define some quantities: 
% %
we measure the extent to which a $k$-clustering~$\mathcal{C}=(C_1,\ldots,C_k)$ of a dataset $\dataset$ is \mbox{(un-)fair} by 
%the two quantities 
$\Nrunf$ (``number unfair'') and $\Maxviol$ (``maximum violation'') defined as
%
\begin{align}\label{exp_quantities_unfair}
\Nrunf=|\{x\in \dataset: \text{$x$ is not treated fair}\}|,~\quad~ \Maxviol=\max_{x\in\dataset} \max_{C_i\neq C(x)}\frac{\frac{1}{|C(x)|-1}
\sum_{y\in C(x)} d(x,y)}{\frac{1}{|C_i|}\sum_{y\in C_i} d(x,y)},
\end{align}
%For the definition of $\Maxviol$ 
where 
we use the convention that $\frac{0}{0}=0$. 
% $\Maxviol$ is the maximum ratio 
% between the average distance of a data point to the points in its own cluster and the 
% average distance of the data point to the points in another cluster.  
% %(where the maximum is over all data points and other clusters).  
% %Note that 
The clustering~$\mathcal{C}$ is fair if and only if
$\Nrunf=0$ and 
%/ or 
$\Maxviol\leq 1$. 
%
%
% 
Mainly 
if $\dataset\subseteq \R^m$ and 
%$d=\|\cdot - \cdot\|_2$. 
$d$ is the Euclidean metric, 
we measure the quality of~$\mathcal{C}$ 
(with respect to 
%(w.r.t. 
the 
%clustering 
goal of putting similar data points into the same cluster) by 
the $k$-means cost, referred to as $\sqcost$ (``cost squared''). In general, we measure the quality of~$\mathcal{C}$ by $\cost$ (``cost''),
which is 
%more
compatible with 
%our definition of individual fairness in 
Definition~\ref{def_indi_fairness} in that it uses ordinary 
%distances 
rather than squared distances as $\sqcost$.  
It is 
\begin{align}\label{exp_cost_sq}
\sqcost =\sum_{i=1}^k \frac{1}{2 |C_i|}\sum_{x,y\in C_i}d(x,y)^2,\qquad  
 \cost =\sum_{i=1}^k \frac{1}{2|C_i|}\sum_{x,y\in C_i}d(x,y).
\end{align}
The reason for 
%also 
using $\sqcost$ as a measure of quality is 
%mainly 
to provide a fair evaluation of $k$-means clustering. 




%
%All experiments were performed 
We performed all experiments  
in Python \textbf{(code in the supplementary material)}. 
We used the 
%implementations of the 
standard clustering algorithms from Scikit-learn or SciPy with all parameters set to their default~values.








\begin{table}[t]
\caption{Experiment on German credit data set. Clustering 1000 people according to their credit amount. Target cluster sizes $t_i=\frac{1000}{k}$, $i\in [k]$. 
%$k$-means initialized with data points $x_{t_1/2},x_{t_1/2+t_1},\ldots,x_{t_1/2+(k-1)t_1}$.  $k$-means++ results are average over 100 runs.
%\textsc{DP}$=$dyn. programming, 
\textsc{$k$-me++}$=k$-means++. 
% Results for 
% \textsc{$k$-me++}  
% %$k$-means++
% averaged over 100 runs. 
Best values in~bold.
}
\label{experiment_1Da}

%\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccccccccccc}
\toprule
 & $\Nrunf$ & $\Maxviol$ & $\Obj$ & $\sqcost$ & $\cost$ && $\Nrunf$ & $\Maxviol$ & $\Obj$ & $\sqcost$ & $\cost$ \\
\midrule
&  \multicolumn{5}{c}{$k=5$} &&  \multicolumn{5}{c}{$k=50$}\\
\addlinespace[0.1cm]
Naive &  105 & 2.95 & \textbf{0} & 4.78 & 23.53 && 101 & 2.6 & \textbf{0} & 0.19 & 3.06\\ 
DP & \textbf{0} & \textbf{1.0} & 172 & 1.39 & 17.62 && \textbf{0} & \textbf{1.0} & 8 & 0.08 & 2.29\\ 
$k$-means~ & 1 & 1.0 & 170 & 1.39 & \textbf{17.61} && 18 & 1.26 & 10 & 0.1 & 2.54\\ 
$k$-me++~& 0.79 & 1.0 & 279 & \textbf{1.38} & 19.36 && 11.04 & 1.15 & 50 & \textbf{0.01} & \textbf{1.72}\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}























\subsection{
%Dynamic Programming Approach for 
1-dimensional 
%1-dim 
Euclidean 
%Case
Data Sets
}\label{section_experiments_1D}

We used the German Credit data set 
%\citep{Dua:2019_German_credit_data}
\citep{UCI_all_four_data_sets_vers2}.  
%for our experiments in the 1-dimensional Euclidean case. 
%This data set 
It 
comprises 1000 records (corresponding to 
%people)
human beings) 
and for each record one binary label (good vs. bad credit risk) and 20 features. 

In our first experiment, we clustered the 1000 people according to 
%the 
their credit amount, which is one of the 20 features.   
A~histogram of the data  
can be seen in 
%the left plot of 
Figure~\ref{plot_histogram_1D_data} in Appendix~\ref{appendix_exp_1dim}. We 
%assumed to aim 
were aiming 
for $k$-clusterings with clusters of equal size (i.e., 
target cluster sizes $t_i=\frac{1000}{k}$, $i\in [k]$) and compared our DP approach of 
Section~\ref{section_1dim} with $p=\infty$ to 
$k$-means clustering 
%and
as well as 
a naive clustering that simply puts the 
%first $t_1$ many 
$t_1$ smallest 
points in the first cluster, the next $t_2$ many points in the second cluster, and so on. 
We considered two initialization strategies for $k$-means:  we either used the medians of the clusters of the naive clustering for initialization 
(thus, hopefully, biasing $k$-means towards the target cluster sizes) or we ran $k$-means++ \citep{kmeans_plusplus}. 
%(the default initialization in Scikit-learn). 
For the latter we report average 
results obtained from running the experiment for 100 times. In addition to the four quantities $\Nrunf$, $\Maxviol$, $\sqcost$ and  $\cost$ defined in 
\eqref{exp_quantities_unfair} and \eqref{exp_cost_sq}, we report $\Obj$ 
(``objective''),  
which is the value of the objective function of 
%the minimization problem~
\eqref{1dim-problem} 
for $p=\infty$. 
Note that $k$-means 
%always 
yields contiguous clusters and 
%hence 
$\Obj$ is meaningful for all four clustering methods that we consider. 


The results are provided in Table~\ref{experiment_1Da} ($k=5$ and $k=50$) and in Table~\ref{experiment_1Da_part2} ($k=10$ and $k=20$) in Appendix~\ref{appendix_exp_1dim}. 
As expected, for the naive clustering we always have $\Obj=0$, 
for our  
%dynamic programming 
DP approach (\textsc{DP}) we have $\Nrunf=0$ and 
$\Maxviol\leq 1$, and $k$-means++ (\textsc{$k$-me++}) performs best in terms of $\sqcost$. 
Most interesting to see is that both versions of $k$-means yield almost perfectly fair clusterings when $k$ is small 
%but $k$-means can yield clusterings that treat up to 18 data points unfair when $k=50$. 
and moderately fair clusterings when $k=50$ (with $k$-means++ outperforming $k$-means). 

In our second experiment (presented in Appendix~\ref{appendix_exp_1dim}), we used the first 500 records 
%of the data set 
to train a multi-layer perceptron (MLP)
%with three hidden layers of size 100, 50 and 20, respectively) 
for predicting the label (good vs. bad credit risk). 
We then 
%used
applied 
the MLP to estimate the probabilities of having a good credit risk for the other 500 people.    
%(the test error of the MLP is 0.276)  
%(the test accuracy of the MLP is 0.724).  
We used the same clustering methods as in the first experiment to cluster 
the 500 people according to their probability estimate. 
We believe that such a clustering problem may arise 
frequently in practice (e.g., when a bank determines its lending policy) and that individual fairness is highly desirable in 
%such a sensitive 
this 
context.  













%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






\subsection{General Data Sets}\label{section_experiments_general}

We performed the same set of experiments on the first 1000 records of the 
Adult data set, the Drug Consumption data set (1885 records), and the Indian Liver Patient data set (579 records) \citep{UCI_all_four_data_sets_vers2}. 
%All three data sets are available on the UCI ML repository \cite{UCI_all_four_data_sets_vers2}. 
%
As distance function~$d$ we  used the Euclidean, 
Manhattan or Chebyshev metric.  
% %based on 
% with respect to
% the features of 
% a
% %the 
% data set.
Here we only present the results for the Adult data set and the Euclidean metric, the other results  are provided in Appendix~\ref{appendix_exp_general}.
Our observations are largely consistent between the different data sets~and~metrics. 
%under consideration.

%\paragraph{First Experiment --- (Un-)Fairness of Standard Algorithms}
%\paragraph{First Experiment: (Un-)Fairness of Standard Algorithms}
\vspace{1mm}
\textbf{First Experiment --- (Un-)Fairness of Standard Algorithms}~~~~Working with  the Adult data set, 
we only used its six numerical features
(e.g., age, hours worked per week), normalized to zero mean
and unit variance, for representing records. 
%
We applied several standard clustering algorithms as well as the group-fair $k$-center algorithm of 
\citet{fair_k_center_2019} (referred to as $k$-center~GF) 
to the data set ($k$-means++; $k$-medoids; spectral clustering (SC)) or its 
distance matrix
%~$(d(x,y))_{x,y\in\dataset}$ 
($k$-center using the greedy strategy of \citet{gonzalez1985}; $k$-center GF; single / average / complete linkage clustering). 
%We ran $k$-center~GF with the constraint of choosing $\lfloor k/2\rfloor$ female and $\lceil k/2\rceil$ male centers. 
%
In order to study the extent to which these methods produce (un-)fair clusterings, for $k=2,5,10,20,30,\ldots,100$, 
we computed 
$\Nrunf$ and $\Maxviol$ as defined in~\eqref{exp_quantities_unfair} for the resulting $k$-clusterings. 
For measuring the quality of the clusterings we computed $\sqcost$ or $\cost$ as defined in~\eqref{exp_cost_sq}.  







\newcommand{\scaleA}{0.275}


\begin{figure*}[t]
\centering
% \includegraphics[width=1\textwidth]{exp_gen_data_sets_AfterRebuttal/AdultData/legend_cropped.pdf}
% 
% \includegraphics[scale=\scaleA]{exp_gen_data_sets_AfterRebuttal/AdultData/AdultData_NrUnf_AsFunctionOfk_n=1000_NrReplicates=25_distance=euclidean_NOLEGEND.pdf}
% \hspace{0mm}
% \includegraphics[scale=\scaleA]{exp_gen_data_sets_AfterRebuttal/AdultData/AdultData_MaxViol_AsFunctionOfk_n=1000_NrReplicates=25_distance=euclidean.pdf}
% \hspace{0mm}
% \includegraphics[scale=\scaleA]{exp_gen_data_sets_AfterRebuttal/AdultData/AdultData_CostSquared_AsFunctionOfk_n=1000_NrReplicates=25_distance=euclidean.pdf}
% 
% %\includegraphics[width=1\textwidth]{exp_gen_data_sets_AfterRebuttal/AdultData/legend_cropped.pdf}
% 
\includegraphics[width=\textwidth]{images_compressed/fig3.pdf}

\vspace{-2mm}
\caption{$\Nrunf$ 
\textbf{(left)}, $\Maxviol$ 
\textbf{(middle)} and $\sqcost$ \textbf{(right)}
for the clusterings produced by the 
various 
%standard 
algorithms as a function of 
%the number of clusters~$k$.
$k$.
}\label{exp_gen_standard_alg_Adult}
\end{figure*}










The results are provided in 
Figure~\ref{exp_gen_standard_alg_Adult}.  
For $k$-means++, $k$-medoids, $k$-center, $k$-center GF and SC we show average results obtained from running 
%these algorithms 
them 
for 
25 times since their outcomes depend on random initializations. 
We can see that, in particular for large values of~$k$, $k$-center, $k$-center GF, SC, and the linkage algorithms can be quite unfair 
%and yield 
with 
rather large values of $\Nrunf$ and $\Maxviol$. 
In contrast, $k$-means++ produces rather fair clusterings with $\Nrunf\leq 90$ and $\Maxviol\leq 1.4$ even when $k$ is large. 
For 
a 
baseline comparison, for a random clustering in which every data point was assigned to one of $k$ clusters uniformly at random we observed 
$\Nrunf= 990$ and $\Maxviol=4.0$ on average (when $k=100$). 
%
The beneficial behavior of $k$-means++ with respect to our notion of individual fairness 
raises the question whether one 
%could actually 
can 
prove guarantees on the extent 
to which clusterings produced by 
$k$-means++ are fair (cf. Section~\ref{section_discussion}). 
%
The $k$-medoids algorithm performs worse than $k$-means++, but better than the other algorithms. The clusterings produced by 
$k$-center~GF, which we ran with the constraint of choosing $\lfloor k/2\rfloor$ female and $\lceil k/2\rceil$ male centers,  
are slightly more fair than the ones produced by $k$-center.
However, note that it really depends on the data set whether~a group-fair 
clustering is individually fair or not (example 
provided 
in Appendix~\ref{example_group_fair_vs_indi_fair}). 
%
Unsurprisingly, $k$-means++ outperforms the other methods in terms of $\sqcost$ since it is designed with 
the~goal~of~minimizing~this~quantity. 










\begin{figure*}[t]
\centering
% \includegraphics[scale=\scaleA]{exp_gen_data_sets_AfterRebuttal/AdultData/AdultDataHEURISTICS_NrUnf_AverageLink_AsFunctionOfk_n=1000_NrReplicates=25_distance=euclidean.pdf}
% \hspace{0mm}
% \includegraphics[scale=\scaleA]{exp_gen_data_sets_AfterRebuttal/AdultData/AdultDataHEURISTICS_MaxViol_AverageLink_AsFunctionOfk_n=1000_NrReplicates=25_distance=euclidean.pdf}
% \hspace{0mm}
% \includegraphics[scale=\scaleA]{exp_gen_data_sets_AfterRebuttal/AdultData/AdultDataHEURISTICS_Cost_AverageLink_AsFunctionOfk_n=1000_NrReplicates=25_distance=euclidean.pdf}
%
\includegraphics[width=\textwidth]{images_compressed/fig4.pdf}

\vspace{-2mm}
\caption{$\Nrunf$ 
\textbf{(left)}, $\Maxviol$ 
\textbf{(middle)} and $\cost$ \textbf{(right)}
for the clusterings produced by average linkage clustering 
and the two variants of our heuristic 
%approach 
to improve it: the first ($\#$U in the legend) greedily chooses splits as to minimize $\Nrunf$, the second 
%(MV in the legend) 
(MV) 
as to minimize $\Maxviol$.
}
\label{exp_gen_heuristics_Adult}
\end{figure*}





%\paragraph{Second Experiment --- Heuristics to Improve Linkage Clustering}
\vspace{1mm}
\textbf{Second Experiment --- Heuristics to Improve Linkage Clustering}~~~~One might wonder whether there are 
%simple 
modifications to the standard clustering algorithms 
%in order to 
that 
make them more fair.  
A natural idea to make any clustering 
% %(and hence 
% (or 
% clustering algorithms) 
more fair is to make local changes to 
%the clustering
it 
%by iteratively picking a data point that is not treated fair and assigning 
and iteratively pick a data point that is not treated fair and assign 
it to the cluster that it is closest too. 
%After the assignment the data point that has been moved is treated fair.
After picking and reassigning a data point, this 
%data 
point is treated fair. However, 
in 
%our 
experiments we observed that  usually we can only pick 
a very small number of data points whose reassignment does not cause other 
%data 
points that are initially treated fair to be treated unfair after the reassignment 
(example provided in Appendix~\ref{example_local_search}). 
%Hence, this idea does not seem to be~useful.

Another idea that we want to present here is specifically tied to linkage clustering. 
As our experiments show this idea results in  linkage clustering producing clusterings that are significantly more fair than the ones produced by ordinary linkage clustering. 
Linkage clustering 
%produces 
builds 
a binary tree that represents a hierarchical clustering with the root of the tree corresponding to the whole data set and 
every 
%vertex 
node 
corresponding to a subset such that a parent is the union of its two children.   
The leaves of the tree correspond to singletons comprising one data point 
\citep[e.g., ][Section 22.1]{shalev2014understanding}. If one wants to obtain a $k$-clustering of the data set, 
the output of a linkage clustering 
algorithm is a certain pruning of this tree.
When individual fairness is a goal, 
we propose to construct a $k$-clustering / a pruning of the tree as follows 
(pseudocode provided in Appendix~\ref{appendix_pruning_strategy}): starting with the two children of the root, 
we maintain a set of 
%vertices
nodes 
that corresponds to a clustering 
and proceed in $k-2$ rounds. In round~$i$, we greedily 
%replace 
split 
one of the $i+1$ many 
%vertices 
nodes 
that we currently have into its two children such that the resulting $(i+2)$-clustering minimizes, over the $i+1$ many possible splits, 
 $\Nrunf$ as defined in 
\eqref{exp_quantities_unfair}. Alternatively, we can split the node that 
%is best with respect to 
gives rise to a minimum value of 
$\Maxviol$ (also defined in \eqref{exp_quantities_unfair}). 




In Figure~\ref{exp_gen_heuristics_Adult}, we show $\Nrunf$, $\Maxviol$ and $\cost$ for ordinary average linkage clustering and a modified version 
using our heuristic approach in its both variants ($\#$U denotes the variant 
%with 
based on
$\Nrunf$ and MV the variant 
%with
based on 
$\Maxviol$). 
Analogous experiments 
with single or complete instead of average linkage clustering are presented 
in Appendix~\ref{appendix_exp_general}. We can see that our 
%heuristic 
approach leads to a 
significant 
improvement in $\Nrunf$ (for $k\leq 50$ this holds for both variants, 
but in particular for the variant 
aiming to minimize $\Nrunf$). The variant 
%aiming at minimzing 
based on 
$\Maxviol$ leads to an improvement in $\Maxviol$. However, these improvements come at the price of an increase in 
$\cost$ as we can see from the right plot of Figure~\ref{exp_gen_heuristics_Adult}.
 




==> Indi Fairness - Arxiv/fairness.tex <==
Our notion of individual fairness 
%for clustering 
applies to a data set~$\dataset$ together 
with a 
given  dissimilarity function~$d$ that measures how 
%(dis-)similar 
close
two data points are. 
%In the following, 
We 
use the terms  dissimilarity and distance synonymously. 
%We denote the data set by $\dataset$ and the dissimilarity function by $d$. 
We assume $d:\dataset\times \dataset\rightarrow\R_{\geq 0}$ to be 
symmetric with $d(x,x)=0$, but not necessarily to 
be a metric (i.e., to additionally satisfy the triangle~inequality and $d(x,y)=0 \Leftrightarrow x=y$).

Our fairness notion defines what it means that a data point is treated fair in a clustering of $\dataset$; namely: 
a data point is treated individually fair if the average distance to the points 
in its own cluster (the point itself excluded) is not greater than the average distance to the points in any other cluster. 
Then 
a clustering 
of $\mathcal{D}$ 
is said to be individually fair if it treats every data point 
of $\mathcal{D}$ 
individually fair. 





\begin{figure}[t]
 \centering
 \includegraphics[scale=0.9]{sketches/fair_annotated.pdf}
 \hspace{3cm}
  \includegraphics[scale=0.9]{sketches/unf_annotated.pdf}


%\vspace{-0pt}
 \caption{Two data sets in $\R^2$ with $d$ equaling the Euclidean metric. \textbf{Left:} An individually fair 3-clustering with clusters $C_1,C_2,C_3$.  
 \textbf{Right:} Four points for which there is no individually fair 2-clustering. For example, if 
 %$\mathcal{C}=(C_1,C_2)$ with 
 the two clusters were 
 $C_1=\{x_1,x_4\}$ and $C_2=\{x_2,x_3\}$, then $x_1$ would be treated unfair because of  
% $d(x_1,x_4)=0.71>0.68=\frac{d(x_1,x_2)+d(x_1,x_3)}{2}$
$d(x_1,x_4)=0.71>0.68=[d(x_1,x_2)+d(x_1,x_3)]/2$.
 }\label{figure_example}
\end{figure}






For the rest of the paper we assume $\dataset$ to be finite. Our definition of individual fairness for clustering can then be formally stated as follows 
(for $l\in\N$, we 
%use
write 
$[l]=\{1,\ldots,l\}$):

\begin{definition}[Individually fair clustering]\label{def_indi_fairness}
 Let $\mathcal{C}=(C_1,\ldots,C_k)$ be a $k$-clustering of $\dataset$, that is 
 $\dataset=C_1\dot{\cup}\ldots\dot{\cup}C_k$ and 
 $C_i\neq \emptyset$ for $i\in[k]$. For $x\in \dataset$, we write $C(x)$ 
 for the cluster $C_i$ that $x$ belongs to. 
 %
 We say that $x\in \dataset$ is 
%\emph{treated individually fair} 
treated individually fair
if either $C(x)=\{x\}$ or
 \begin{align}\label{def_individual_fairness_ineq}
\frac{1}{|C(x)|-1}
%\sum_{y\in C(x)\setminus\{x\}} 
\sum_{y\in C(x)} 
d(x,y)\leq \frac{1}{|C_i|}\sum_{y\in C_i} d(x,y) 
 \end{align}
for all $i\in[k]$ with $C_i\neq C(x)$. The clustering $\mathcal{C}$ is 
%\emph{individually fair} 
individually fair
if every $x\in \dataset$ is treated individually fair.\footnote{For brevity, when it is clear from the context, instead of 
``individually fair'' we may only say ``fair''.}
\end{definition}







\begin{figure}[t]
\centering
\hspace{-6mm}\begin{overpic}[scale=0.24,trim=80 80 80 80,clip]{sketches/example_1D_newA_mod}
 \put(21,1.2){$8$}
\put(51,1.2){$1$}
\put(38.3,0.6){\small $\frac{1}{3}$}
\put(81,1.2){$8$}
\put(108,12.5){\includegraphics[scale=0.25]{sketches/separator2.pdf}}
 \end{overpic}
 \hspace{2mm}
 \includegraphics[scale=0.24,trim=80 80 100 80,clip]{sketches/example_1D_new_mod}
 
 %\vspace{-3pt}
 \caption{An example of a data set 
 %with $10$ points 
 on the real line with more than one individually fair clustering. \textbf{Left:} The data set and the distances between the points. 
 \textbf{Right:} The same data set with two 
 fair 
 2-clusterings (one encoded by color: red vs blue / one encoded by frames: solid vs dotted boundary).
 %, both of which are fair.
 }\label{figure_example_2}
\end{figure}






We 
%want to 
discuss some important observations about individually fair clusterings as defined in Definition~\ref{def_individual_fairness_ineq}: 
if in a clustering all clusters are well-separated and sufficiently far apart, 
then this clustering is 
%individually 
fair. 
An example of such a scenario is provided in the left part of Figure~\ref{figure_example}. 
Hence, at least for such  simple clustering problems
with an ``obvious'' solution, 
individual fairness does not conflict with the clustering 
goal of
%to partition 
partitioning 
the data set  
%in such a way that 
such that 
``data points in the same cluster are similar to each other, and data points in different clusters are dissimilar'' \citep[][p.~306]{celebi2016}.
%
However, there are 
also 
%some 
data sets for which no 
%individually 
fair $k$-clustering exists 
%at all 
(for a fixed~$k$ 
and a given distance function~$d$).\footnote{
Of course, the trivial $1$-clustering $\mathcal{C}=(\dataset)$ or  
the 
trivial $|\dataset|$-clustering that puts every 
data 
point in a singleton are 
%always 
fair, 
and for a trivial distance function~$d\equiv 0$, every clustering is fair.
}
This can even happen for Euclidean data sets and $k=2$, as the right part of Figure~\ref{figure_example} shows.
If a data set allows 
for an individually fair $k$-clustering, there might be more than one fair $k$-clustering. An example of this is
shown in 
Figure~\ref{figure_example_2}. This example 
also 
illustrates 
that 
individual fairness does not necessarily work towards the 
aforementioned 
clustering 
goal.  
Indeed, in Figure~\ref{figure_example_2} the 
two 
clusters of the  clustering encoded by the frames, which is 
%individually 
fair,  are not even~contiguous.  

These observations raise 
a 
%great 
number 
%several 
of questions such as: when does 
%an individually 
a 
fair $k$-clustering exist? Can we efficiently decide whether a fair $k$-clustering exists? 
If a fair $k$-clustering exists, can we efficiently compute it? Can we minimize some (clustering) objective 
%such as the $k$-means cost 
over the set of all 
%individually 
fair clusterings? If no fair $k$-clustering exists, can we find a clustering that violates inequality~\eqref{def_individual_fairness_ineq} only for a few data points, or 
a clustering that potentially violates \eqref{def_individual_fairness_ineq} for every data point, but only to a minimal extent? How do standard clustering algorithms such as 
Lloyd's algorithm (aka $k$-means) 
or linkage clustering \citep[e.g.,][Section 22]{shalev2014understanding}
perform in terms of 
%individual 
fairness? Are there simple modifications to these 
algorithms 
in order to 
%that 
%%can  
improve their~fairness?
%
In this paper, we explore some of these questions as outlined 
%already 
in Section~\ref{section_introduction}. 
%
%Before presenting our contributions, we discuss related work and concepts in the following subsection.





\subsection{Related Work and Concepts}\label{sec_related_work_and_concepts}

We provide a detailed overview in Appendix~\ref{appendix_related_work}. Here we only present a brief summary.

%\paragraph{Existing Notions of Individual Fairness}
\textbf{Existing Notions of Individual Fairness}~~~
\citet{fta2012} were the first to provide a notion of individual fairness by asking that 
similar data points (as measured by a given task-specific metric) should be treated
similarly by a randomized classifier. Subsequently, individual fairness has been studied in multi-armed bandit problems  
\citep{joseph2016,joseph2018,gillen2018}. 
%
The recent work of \citet{kearns_average_individual_fairness} 
% studies the scenario that every individual is subject to a 
% %number 
% multitude 
% of classification tasks and 
introduces the notion of average individual fairness. 


%\paragraph{Fairness for Clustering}
%\vspace{1mm}
\textbf{Fairness for Clustering}~~~~The most established notion of fairness for clustering has been proposed by 
\citet{fair_clustering_Nips2017}. 
It asks that
each cluster has proportional representation from different
demographic groups. 
Several follow-up works extend 
that work 
\citep{roesner2018,sohler_kmeans,ahmadian2019,anagnostopoulos2019,backurs2019,bera2019,bercea2019,huang2019,fair_SC_2019,davidson2020}.

Alternative fairness notions for clustering 
are
tied to centroid-based clustering such as $k$-means, $k$-center and $k$-median
\citep{fair_k_center_2019,chen2019,jung2020}.
The recent notion of  
\citet{jung2020}  is the only one that comes with a guarantee for every single data point. It asks that every data point is 
somewhat close to a center, where ``somewhat'' depends on how close the data point is to its $k$ nearest neighbors 
and the motivation
for this notion 
comes from facility location. 
 

%\paragraph{Average Attraction Property}
%\vspace{1mm}
\textbf{Average Attraction Property and Game-theoretic Interpretation}~~~~Our notion of individual fairness is closely related to the 
 average attraction property studied by \citet{vempala2008}, and our notion also has a game-theoretic interpretation.

==> Indi Fairness - Arxiv/introduction.tex <==


Clustering is a classic unsupervised learning procedure 
and is
used in a wide range of fields to understand which data points are most
similar to each other, which regions in space a data set inhabits with
high density~\citep{ester1996density}, 
or 
%and 
to select representative
elements of a data set 
%on which to do preliminary data analysis
\citep{hastie2009}. The problem of clustering can be formulated 
%and studied 
in 
%many 
numerous 
ways, including objective-based formulations like
$k$-median \citep{awasthi2014center}, hierarchical
partitionings \citep{dasgupta2002performance}, and spectral clustering
\citep{Luxburg_tutorial}, which have also been considered subject to
additional constraints~\citep{wagstaff2001constrained}. A
recent surge in work has designed clustering algorithms to satisfy
various notions of proportional representation, including
proportionality for different demographics within
clusters~\citep{fair_clustering_Nips2017} or within the set of cluster
centers \citep{fair_k_center_2019}, or requiring a notion of
coherence on large subsets of a cluster~\citep{chen2019}.



All the latter  
proportionality constraints 
%for clustering 
fall into the category of {\em group fairness}
constraints~\citep{friedler2016possibility}, which 
require a model to have similar statistical behavior for different
demographic groups. Such statistical guarantees necessarily give no
guarantee for any particular individual. For example, while profiles
of women might be equally represented in different clusters,  
such a clustering might not be a good clustering for any particular woman.
%
This weakness of proportionality constraints raises a natural
question: can one construct clusterings that provide fairness
guarantees for each individual,  
%data point, 
and what kind of fairness guarantees 
would an individual want to have after all? 


We 
argue 
that if a clustering is used in a machine learning downstream task, then rather than  
caring about fairness of the clustering, one should care about fairness at the end of the pipeline and 
tune the clustering accordingly. This is analogous to using clustering as a preprocessing step for classification 
and caring about accuracy \citep{luxburg_ScienceOrArt}. However, if a clustering is used by a human decision maker, 
say for exploratory data analysis or resource allocation, an individual 
may strive for being well represented, which means  to be assigned to a cluster with similar data points. 
As a toy example, think of a company that clusters its customers and distributes semi-personalized coupons, where all customers 
in one cluster get the same coupons 
according to 
their 
(hypothesized)
preferences. 
A customer that ends up in a cluster with rather different other customers 
(and hence is not well represented by its cluster)
might get coupons that are less valuable to her than the 
%ones 
coupons 
she would have got 
if she had been assigned to the 
%best representing~cluster.  
cluster that is best representing her. 



Motivated by such an example, 
our notion of individual fairness asks that each data point is assigned to the best representing cluster in the sense 
that the data
point, on average, is closer to the points~in its own
cluster than to the points in any other cluster.
 While our notion is related to a well-known concept of
clustering stability 
%\citep{vempala2008},
(cf. Section~\ref{sec_related_work_and_concepts}), 
many 
%fundamental 
questions
%remain unanswered.
are open. 
For instance, 
in contrast to the existing group fairness notions, 
an {\indf} clustering may not
%necessarily 
exist (for a fixed number of clusters).
%
%In this work, 
We make the following contributions towards
understanding 
{\indfn}~for~clustering:
\begin{itemize}[wide, labelwidth=!, labelindent=0pt]
\setlength{\itemsep}{-0.2pt}

\item We propose a natural notion of {\indfn} for clustering requiring 
%that each
that every 
data point, on average, is closer to the points in its own
cluster than to the points in any other cluster.
\item When the data lies on the real line, we show that an {\indf} clustering always
  exists, and we design an 
  efficient algorithm to find one.
  We 
  argue  why this 1-dim case 
  is interesting on its own.
\item We show that even for Euclidean data sets in $\R^2$,
  {\indf} clusterings might not exist 
  %Furthermore, we 
  and 
  prove that the
  problem of deciding whether a given data set has an {\indf}
  $k$-clustering is NP-hard, even for $k=2$ 
  and when the underlying distance function is assumed to be a metric.
\item We perform experiments on real data sets and compare the performance of our
  polynomial time algorithm for the 1-dim case with $k$-means clustering. In the case of higher dimensions, we investigate several 
  standard clustering algorithms 
  with respect to our fairness notion.
  

\end{itemize}




==> Indi Fairness - Arxiv/np.tex <==
In this section we present one of the main results of our paper, stating the NP-hardness of deciding whether an individually fair $k$-clustering exists. 
For such a result, 
it is 
%important 
crucial 
to 
specify
%make clear 
how an input instance is encoded: we assume that a data set~$\dataset$ together with a distance function~$d$  
is 
%given in form of 
represented by 
the distance matrix~$(d(x,y))_{x,y\in\dataset}$. 
Under this assumption we can prove  
the following~theorem:


\begin{theorem}[NP-hardness of individually fair clustering]\label{theorem_hardness}
Deciding whether a data set~$\dataset$ together with a distance function~$d$ has an individually fair $k$-clustering 
(for a given parameter $k$) 
is NP-hard. This even holds if $k=2$ is fixed and 
$d$ is required to be a metric.   
\end{theorem}

 
The proof of Theorem~\ref{theorem_hardness} is provided in Appendix~\ref{proof_hardness}. 
%In order to show NP-hardness of the individually fair clustering decision problem we construct
It shows NP-hardness 
of the individually fair clustering decision problem
via a reduction from a variant of 3-SAT. In this variant, we can assume a 3-SAT instance  
to have the 
same number of clauses as number of variables and that each variable occurs in at most three clauses. Given such a formula 
$\Phi=C_1 \wedge C_2\wedge \ldots \wedge C_n$ over variables $x_1,\ldots,x_n$, we construct a metric space~$(\dataset,d)$ with  
%on 
$\dataset=\{True, False,\star,\infty,C_1,\ldots,C_n,x_1,\neg x_1,\ldots,x_n,\neg x_n\}$ such that $\Phi$ is satisfiable if and only if 
%the metric space
$\dataset$ 
has an individually fair 2-clustering. 
The difficult part is in defining 
an appropriate metric 
%a metric 
$d$ 
%on $\dataset$ 
to accomplish this. 


Unless $\text{P}=\text{NP}$, Theorem~\ref{theorem_hardness} implies that 
for general data sets, even when being guaranteed that a fair $k$-clustering exists, 
there cannot be any efficient algorithm for computing such a fair clustering. 
%
However, as with all NP-hard problems, there are two possible remedies: first, we can restrict our considerations to data sets with some special structure. This is what we do 
in 
%the following 
Section~\ref{section_1dim}, where we show that for 1-dimensional Euclidean data sets fair clusterings always exist and can be computed in polynomial time. 
%It is 
We consider it to be 
an interesting question for follow-up work whether one can identify other classes of data sets with such a property (cf. Section~\ref{section_discussion}). 
Second, we can look at approximate versions of individual fairness in which we allow inequality~\eqref{def_individual_fairness_ineq} 
to be violated for a certain number of 
points or where we relax inequality~\eqref{def_individual_fairness_ineq} by introducing a multiplicative factor~$\gamma>1$ on its 
%right-hand 
right 
side. 
We start exploring this direction in our experiments in Section~\ref{section_experiments_general}.






\section{1-dimensional Euclidean Case}\label{section_1dim}

%As discussed in Section~\ref{section_np_hardness}, 
One way to 
%overcome 
cope with the NP-hardness of the individually fair clustering problem is to 
restrict our considerations to data sets with some special structure. 
As an important example, 
%In this section 
here
we study the 
special 
case
of 
$\dataset\subseteq \R$ and $d$ being 
the 
%ordinary 
Euclidean metric. 
We first show that in this case, for any $1\leq k\leq |\dataset|$, 
%an individually 
a 
fair $k$-clustering always exists.
In fact, 
we show that there 
%always 
exists 
%an individually 
a 
fair $k$-clustering with contiguous clusters. By contiguous clusters we mean that 
if $\dataset=\{x_1,\ldots,x_n\}$ with $x_1\leq x_2\leq \ldots\leq x_n$, 
the clustering is 
of the form $\mathcal{C}=(\{x_1,\ldots,x_{i_1}\},\{x_{i_1+1},\ldots,x_{i_2}\},\ldots,\{x_{i_{k-1}+1},\ldots,x_{n}\})$ 
for some $1\leq i_1<i_2<\ldots<i_{k-1}<n$. 
It might be surprising at a first glance that there also exist 
%individually 
fair 
clusterings 
of 1-dimensional data sets 
with non-contiguous clusters, 
and indeed this seems to happen 
%rather 
rarely, but it can happen as the example provided in Figure~\ref{figure_example_2} shows. 
%
%Next
Subsequently, 
we provide an 
%efficient algorithm based on dynamic programming 
efficient dynamic programming (DP) approach 
that finds 
%an individually 
a 
fair $k$-clustering solving
\begin{align}\label{1dim-problem}
 \min_{\substack{\mathcal{C}=(C_1,\ldots,C_k):~\mathcal{C}~\text{is a fair clus-}\\ \text{tering of $\dataset$ with contiguous clusters}}} \|(|C_1|-t_1,\ldots,|C_k|-t_k)\|_p,
\end{align}
where $t_1,\ldots,t_k\in[n]$ with $\sum_{i=1}^k t_i=n$ are 
%some 
given target cluster sizes, $p\in\R_{\geq 1}\cup\{\infty\}$ and $\|\cdot\|_p$ denotes the $p$-norm.


We believe that the results of this section are interesting on its own.
%The results of this section might be interesting on its own.
As 
%a motivating 
an 
example consider the scenario that a teacher wants to give grades 
 based on the number of points that a student obtained 
 %in a course 
 by setting some threshold values (e.g., a student gets a B 
if her number of points is in between 75 and~90). 
%smaller than~90, but not smaller than 75).
This can be interpreted as a 1-dim clustering problem, where clusters have to be contiguous and 
%in this clustering problem 
 individual fairness seems to be a highly desirable goal. Furthermore, 
 some teachers aim for a certain grade distribution (aka grading on a curve), in which case the problem 
 %could 
 can 
 be phrased in the form of \eqref{1dim-problem}.
 %
Clearly, one 
% It is not hard to 
 can 
 think of similar examples in the context of credit scores or recidivism~risk~scores.

Let us now present our technical results 
%(all proofs can be found in Appendix~\ref{proof_existence}). 
(proofs  in Appendix~\ref{proof_existence}). 
A key observation is that a clustering with contiguous clusters is fair if and only if the boundary points of the clusters 
%(i.e., the smallest and largest points of the clusters) 
are treated fair:

\begin{lemma}[Fair boundary points imply fair clustering]\label{lemma_boundary_points}
 Let $\mathcal{C}=(C_1,\ldots,C_k)$ be a $k$-clustering of $\dataset=\{x_1,\ldots,x_n\}$, where $x_1\leq x_2\leq\ldots\leq x_n$, with contiguous clusters 
 $C_1=\{x_1,\ldots,x_{i_1}\},C_2=\{x_{i_1+1},\ldots,x_{i_2}\},\ldots,C_k=\{x_{i_{k-1}+1},\ldots,x_n\}$, for some 
 %$1\leq i_1<i_2<\ldots<i_{k-1}<n$. 
 $1\leq i_1<\ldots<i_{k-1}<n$. Then 
 $\mathcal{C}$ is 
 individually 
 fair if and only if 
all points $x_{i_l}$ and $x_{i_l+1}$, $l\in[k-1]$,
 are treated 
 %individually 
 fair. 
 %
 Furthermore, 
$x_{i_l}$ ($x_{i_l+1}$, resp.) is treated fair if and only if its average distance to the points in $C_l\setminus\{x_{i_l}\}$ ($C_{l+1}\setminus\{x_{i_l+1}\}$, resp.) 
is not greater than the average distance to the points in $C_{l+1}$ ($C_{l}$, resp.). 
\end{lemma}

%The proof of Lemma~\ref{lemma_boundary_points} is elementary and can be found in Appendix~\ref{proof_existence}.
The next theorem states that an individually fair $k$-clustering with contiguous clusters always exists.

\begin{theorem}[Existence of individually fair $k$-clustering]\label{lemma_existence_1D}
 Let  $\dataset\subseteq \R$ and $d$ be the Euclidean metric. 
 For any 
%$k\in[|\dataset|]$ 
$k\in\{1,\ldots,|\dataset|\}$,  
 there exists an individually fair $k$-clustering of $\dataset$ with contiguous clusters.
\end{theorem}

%The proof of Theorem~\ref{lemma_existence_1D} is presented in Appendix~\ref{proof_existence}. 
The proof of Theorem~\ref{lemma_existence_1D} is constructive and provides an algorithm to compute a fair $k$-center 
clustering with contiguous clusters. This algorithm works by maintaining $k-1$ 
%thresholds, 
boundary indices, 
%which encode a clustering, 
corresponding to a clustering
with contiguous clusters, 
and repeatedly increasing these 
%thresholds 
indices until a fair 
clustering is found. We prove that at the 
%very 
latest when no 
%threshold 
index 
can be increased anymore, a fair clustering must have been found. 
However, the running time of the algorithm  scales exponentially with $k$. 

% 
To overcome 
%the exponential running time, 
this, 
in the following we propose an efficient DP approach to find 
%an individually 
a 
solution~to~\eqref{1dim-problem}. 
Let 
%us assume that 
$\dataset=\{x_1,\ldots,x_n\}$ with $x_1\leq \ldots\leq x_n$. 
Our approach builds a 
%table~$T\in(\R_{\geq 0}\cup\{\infty\})^{n\times n\times k}$
table~$T\in(\N\cup\{\infty\})^{n\times n\times k}$
with  
\begin{align}\label{definition_table_T}
T(i,j,l)=\min_{(C_1,\ldots,C_l)\in\mathcal{H}_{i,j,l}} \|(|C_1|-t_1,\ldots,|C_l|-t_l)\|_p^p
\end{align}
for $i\in[n]$, $j\in[n]$, $l\in[k]$, where
\begin{align*}
&\mathcal{H}_{i,j,l}=\big\{\mathcal{C}=(C_1,\ldots,C_l):~\text{$\mathcal{C}$ is a fair $l$-clustering of $\{x_1,\ldots,x_i\}$ with $l$ non-empty}\\
&~~~~~~~~~~~~~~~~~~~~~\text{contiguous clusters such that the right-most cluster $C_l$ contains exactly $j$ points}\big\}
\end{align*}
and $T(i,j,l)=\infty$ if $\mathcal{H}_{i,j,l}=\emptyset$. Here, we consider the case $p\neq \infty$. The modifications of our approach 
%for 
to 
the case~$p=\infty$ are minimal and 
are 
described in 
Appendix~\ref{appendix_p_equals_infty}. 

%Clearly,
The optimal value of \eqref{1dim-problem} is given 
by $\min_{j\in[n]} T(n,j,k)^{1/p}$. Below, we will describe how to use the table~$T$ to compute an individually fair $k$-clustering solving \eqref{1dim-problem}. 
First, we explain how to build $T$. 
%
We have, for $i,j\in[n]$, 
% \begin{align*}
%  T(i,i,1)=|i-t_1|^p~~\text{and}~~T(i,1,i)=\sum_{s=1}^i|1-t_s|^p
% \end{align*}
% for $i\in[n]$
\begin{align}\label{table_T_initial}
\begin{split}
 &T(i,j,1)=\begin{cases}
 |i-t_1|^p,& j=i, \\
 \infty, &j\neq i\\           
           \end{cases},
\qquad
T(i,j,i)=\begin{cases}
 \sum_{s=1}^i|1-t_s|^p,& j=1, \\
 \infty, &j\neq 1\\           
           \end{cases},\\
%
 &T(i,j,l)=\infty,\quad j+l-1>i,
 \end{split}
\end{align}
and
 the recurrence relation, for $l>1$ and $j+l-1\leq i$,
% \begin{align*}
% & T(i,j,l)=\\
%  %
%  &\min_{\substack{~~\\~~\\
%  s\in[i-j-(l-2)]:~ T(i-j,s,l-1)<\infty~\text{and} \\
% %x_{i-j}~\text{is closer to}~\{x_{i-j-s+1},\ldots,x_{i-j-1}\}~\text{than to}~\{x_{i-j+1},\ldots,x_i\}~\text{and}\\
% \frac{1}{s-1}\sum_{f=1}^{s-1}|x_{i-j}-x_{i-j-s+f}|\leq\frac{1}{j}\sum_{f=1}^{j}|x_{i-j}-x_{i-j+f}|~\text{and}\\
% %x_{i-j+1}~\text{is closer to}~~\{x_{i-j+2},\ldots,x_i\}~\text{than to}~\{x_{i-j-s+1},\ldots,x_{i-j}\}}} |t_l-j|^p+T(i-j,s,l-1).
% \frac{1}{j-1}\sum_{f=2}^{j}|x_{i-j+1}-x_{i-j+f}|\leq\frac{1}{s}\sum_{f=1}^{s}|x_{i-j+1}-x_{i-j-s+f}|}}\hspace{-3cm}|t_l-j|^p+T(i-j,s,l-1).
% \end{align*}
\begin{align}\label{recurrence_relation}
\begin{split}
T(i,j,l)=|j-t_l|^p+\min\left\{T(i-j,s,l-1):  s\in[i-j-(l-2)],\frac{\sum_{f=1}^{s-1}|x_{i-j}-x_{i-j-f}|}{s-1}\leq\right.\\
 \left.\frac{\sum_{f=1}^{j}|x_{i-j}-x_{i-j+f}|}{j},\frac{\sum_{f=2}^{j}|x_{i-j+1}-x_{i-j+f}|}{j-1}\leq\frac{\sum_{f=0}^{s-1}|x_{i-j+1}-x_{i-j-f}|}{s}\right\},
\end{split}
\end{align}
where we use the convention that $\frac{0}{0}=0$ for the 
%two 
fractions on the left sides of the inequalities. 
%
We explain the recurrence relation~\eqref{recurrence_relation} and argue why it is correct in Appendix~\ref{appendix_p_equals_infty}.


It is not hard to see that using~\eqref{recurrence_relation}, we can build the table~$T$ in 
%running 
time $\mathcal{O}(n^3k)$. Once we have $T$, we 
can compute a solution $(C_1^*,\ldots,C_k^*)$ to \eqref{1dim-problem} by specifying 
$|C_1^*|,\ldots,|C_k^*|$ 
in 
%running 
time $\mathcal{O}(nk)$ as follows: let $v^*=\min_{j\in[n]} T(n,j,k)$. We set $|C_k^*|=j_0$ for an arbitrary 
$j_0$ with $v^*=T(n,j_0,k)$. For $l=k-1,\ldots,2$, we then set $|C_l^*|=h_0$ for an arbitrary $h_0$~with 
%
(i) $T(n-\sum_{r=l+1}^k |C_r^*|,h_0,l)+\sum_{r=l+1}^k ||C_r^*|-t_r|^p=v^*$,
 (ii) the average distance of $x_{n-\sum_{r=l+1}^k |C_r^*|}$ to the closest $h_0-1$ many  points on its left side is not greater than the average 
distance to the points in $C_{l+1}^*$, and 
(iii) the average distance of $x_{n-\sum_{r=l+1}^k |C_r^*|+1}$ to the other points in $C_{l+1}^*$ is 
 not greater than the average distance to the closest $h_0$ many points on its left side. 
%
Finally, it is $|C_1^*|=n-\sum_{r=2}^k |C_r^*|$. It follows from the definition 
of the table~$T$ in~\eqref{definition_table_T} and Lemma~\ref{lemma_boundary_points} that for $l=k-1,\ldots,2$ we can always find some $h_0$ satisfying (i)~to~(iii)
and that our approach yields an individually fair $k$-clustering $(C_1^*,\ldots,C_k^*)$ of $\dataset$. 

Hence we have shown the following theorem:

\begin{theorem}[Efficient 
%dynamic programming 
DP 
approach solves \eqref{1dim-problem}]
By means of the dynamic programming approach \eqref{definition_table_T} to \eqref{recurrence_relation} we can compute 
an individually 
%a 
fair clustering 
solving 
\eqref{1dim-problem} in running time $\mathcal{O}(n^3k)$.
\end{theorem}



==> Indi Fairness - Arxiv/related_work.tex <==
\section{Related Work and Concepts}\label{appendix_related_work}

\paragraph{Existing Notions of Individual Fairness}

As 
%already 
discussed in Section~\ref{section_introduction}, the existing notions of fairness in 
ML, in particular in the context of classification, can largely be categorized into  group fairness and individual fairness.  
There is also a recent line of work on 
the notion of 
\emph{rich subgroup fairness} \citep{Hebert2018,kearns_2018_subgroup1,kearns_2018_subgroup2,kim2019}, 
which 
%in a way  
falls between these two categories
in that it requires some statistic to be similar 
for a \emph{large} (or even infinite) number of subgroups. Here we focus on the work strictly falling into the category of individual fairness. 

\citet{fta2012} were the first to provide a notion of individual fairness by asking that 
similar data points (as measured by a given task-specific metric) should be treated
similarly by a randomized classifier. 
%
\citet{joseph2016} and \citet{joseph2018} study fairness in multi-armed bandit problems. Their fairness notion  
 aims at guaranteeing fairness on the individual level by asking that in any round, an arm with a higher expected reward 
 %(e.g., 
 (corresponding to a better qualified applicant, 
 for example) 
 is more likely to be played than an arm with a lower expected reward. 
%
Specifically in the contextual bandit setting, \citet{gillen2018} 
 apply the  principle of \citeauthor{fta2012} by requiring that in any round, 
 similar contexts are 
 picked  with approximately equal probability. 
%
The recent work of \citet{kearns_average_individual_fairness} studies the scenario that every individual is subject to a 
%number 
multitude 
of classification tasks 
and introduces the notion of average individual fairness. It asks that all individuals are classified with the same accuracy \emph{on average} over all classification~tasks. 


\paragraph{Fairness for Clustering}

The most established notion of fairness for clustering has been proposed by 
\citet{fair_clustering_Nips2017}. 
It is based on the fairness notion of disparate impact
\citep{feldman2015}, which says that the output of a 
%machine learning 
ML 
algorithm should be independent of a sensitive attribute, and 
asks that
each cluster has proportional representation from different
demographic groups.
\citeauthor{fair_clustering_Nips2017}
provide approximation algorithms that incorporate
their
%this fairness
notion 
into
%for 
$k$-center and $k$-median clustering, assuming that there are only two 
demographic 
groups. 
Several follow-up works extend this line of work to other 
clustering objectives such as $k$-means or spectral clustering, 
multiple or non-disjoint groups, 
some variations of the fairness notion  
or to address scalability issues \citep{roesner2018,sohler_kmeans,ahmadian2019,anagnostopoulos2019,backurs2019,bera2019,bercea2019,huang2019,fair_SC_2019}. 
The recent work of \citet{davidson2020} shows that for two groups, when given any clustering, one can efficiently compute the fair clustering 
(fair according to the notion of \citeauthor{fair_clustering_Nips2017})
that is most similar to the given clustering  
%via 
using 
linear programming.
\citeauthor{davidson2020} also show that it is NP-hard to decide whether a data set allows for a fair clustering that 
%also 
additionally 
satisfies some given must-link constraints.
%\citep{}
They mention that such must-link constraints could be used for encoding individual level fairness constraints of the form ``similar data points must go to the same cluster''. 
However, for such a notion of individual fairness it remains unclear which pairs of data points exactly should be subject to a must-link constraint.



% There are two alternative fairness notions for clustering, 
% both of them tied to centroid-based clustering such as $k$-means, $k$-center and $k$-median, 
% where one chooses $k$ centers and then forms clusters by assigning every data point to its closest center: 
Three 
%existing 
alternative fairness notions for clustering 
are
tied to centroid-based clustering such as $k$-means, $k$-center and $k$-median, 
 where one chooses $k$ centers and then forms clusters by assigning every data point to its closest center.
%motivated 
(i) Motivated 
by the 
application of 
%%use in 
%use case of 
data summarization, \citet{fair_k_center_2019} propose 
that the various demographic groups should be 
proportionally represented among 
the chosen centers.  
(ii) \citet{chen2019} propose a notion of proportionality that requires that 
% there is no sufficiently large subset of data points that 
% could jointly reduce their distances from their corresponding center by choosing a new center.   
no sufficiently large subset of data points could jointly reduce 
%all 
their distances from their 
%corresponding 
closest 
centers by choosing a new center.   
The latter notion is similar to our notion of individual fairness in that it 
assumes that an individual data point 
%aspires 
strives 
to be well represented (in the notion of \citeauthor{chen2019} by being close to a center). Like our notion and other than the fairness notions of 
\citet{fair_clustering_Nips2017} and \citet{fair_k_center_2019}, it does not rely on demographic group information. 
However, while our notion aims at ensuring fairness for every single data point, the notion of \citeauthor{chen2019} only looks at sufficient large subsets. Furthermore, 
since our notion defines 
%the quality of representation of a data point $x$ by the average distance of $x$ to the points in $x$'s cluster, 
``being well represented'' in terms of the average distance of a data point to the other points in its cluster, 
our notion is not restricted to centroid-based clustering.
%
%Finally, 
(iii) Only recently, 
\citet{jung2020}  proposed a notion of individual fairness for centroid-based clustering that comes with a guarantee for every single data point. It asks that every data point is 
somewhat close to a center, where ``somewhat'' depends on how close the data point is to its $k$ nearest neighbors. Building on the work of \citeauthor{jung2020}, \citet{mahabadi2020} proposed a local search based algorithm 
for this fairness notion that comes with constant factor approximation guarantees.





\paragraph{Average Attraction Property}

\citet{vempala2008} study which properties of a similarity function are sufficient in order to approximately recover 
(in either a list 
%model 
or a tree model) 
%an underlying 
an unknown 
ground-truth clustering. One of the weaker properties they consider is 
%what they call 
the  average attraction property, 
which is 
%essentially the same as 
closely related to 
our notion of individual fairness and requires inequality~\eqref{def_individual_fairness_ineq} to hold 
for the ground-truth clustering 
with 
an additive 
%offset 
gap of~$\gamma>0$ between the 
%left- and the right-hand side 
left and the right side 
of 
%the inequality.
\eqref{def_individual_fairness_ineq}. 
\citeauthor{vempala2008} show that the average attraction property is 
sufficient to successfully cluster in the list model, but with the length of the list 
%depending exponentially on $1/\gamma$,  
being exponential in $1/\gamma$, 
and is not sufficient to successfully cluster in the tree model.
%
The conceptual difference between the work of \citeauthor{vempala2008} and 
%our paper 
ours 
is that the 
former assumes a ground-truth clustering and considers the 
average attraction property as a helpful property 
%of the similarity function 
to find this ground-truth clustering, while we consider individual fairness as a constraint we would 
like to impose on whatever clustering~we~compute.



\paragraph{Game-theoretic Interpretation}

Fixing the number of clusters~$k$, 
our notion of an individually fair clustering can be interpreted in terms of a 
%particular 
strategic game:   
%where
let 
each data point 
%corresponds 
correspond 
to a player that can play an action in $[k]$ in order to determine which cluster it belongs to. If, upon the cluster choice of each player,
a data point is treated fair according to Definition~\ref{def_indi_fairness}, this data point gets a utility value of $+1$; otherwise it gets a utility value of $0$. 
%In this setting, 
Then 
a clustering is individually fair if and only if it is a pure (strong / Pareto) Nash equilibrium of this 
particular 
game. It is well-known 
for many games 
that deciding whether the game has a pure Nash equilibrium is NP-hard \citep{gottlob2005}. However, none of the existing 
%game-theoretic 
NP-hardness results in game theory 
implies NP-hardness of 
%our particular game.
individually fair clustering.

